Stochastic Games with Disjunctions of Multiple Objectives (Technical Report)

Stochastic games combine controllable and adversarial non-determinism with stochastic behavior and are a common tool in control, verification and synthesis of reactive systems facing uncertainty. Multi-objective stochastic games are natural in situations where several - possibly conflicting - performance criteria like time and energy consumption are relevant. Such conjunctive combinations are the most studied multi-objective setting in the literature. In this paper, we consider the dual disjunctive problem. More concretely, we study turn-based stochastic two-player games on graphs where the winning condition is to guarantee at least one reachability or safety objective from a given set of alternatives. We present a fine-grained overview of strategy and computational complexity of such \emph{disjunctive queries} (DQs) and provide new lower and upper bounds for several variants of the problem, significantly extending previous works. We also propose a novel value iteration-style algorithm for approximating the set of Pareto optimal thresholds for a given DQ.

==> 3c_CQ_determ.tex <==
While SG are generally not determined for CQs or DQs (see \cite{cfk13} or our example in the introduction), it may still be the case that determinacy holds for a specific given game and query.
The theme of this section is to prove (or disprove) determinacy in such cases.
To this end, we devise a sufficient criterion making it surprisingly easy to certify determinacy of several sub-classes of SGs (Section~\ref{sec:determSufficientCondition}).
On the other hand, we show how an algorithm from~\cite{lics-mosg} can be employed in a general decision procedure (Section~\ref{sec:determDecProc}).

\subsection{Sufficient condition for determinacy}\label{sec:determSufficientCondition}

%\begin{theorem}
%    \todot{this is new, I will still reformulate this}
%    Let $Q = \{q \mid \exists s \in \Sprob \colon p(s,t)=q \}$ be the probabilities occurring in $\game$. Let $\pcurves' \subseteq \pcurves$ be closed under convex unions, intersections and weighted sums $qX_1 + (1-q)X_2$. Further suppose that the following distributive laws hold for all $X, X_1, X_2 \in \pcurves'$
%    \begin{itemize}
%        \item $\conv(X \cup X_1) \cap \conv(X \cup X_2) = \conv(X \cup (X_1 \cap X_2))$
%        %        \item
%        %        $(qX + (1-q)X_1) \cap (qX + (1-q)X_2) = qX + (1-q)(X_1 \cap X_2)$ (I think is trivial)
%    \end{itemize}
%    Let $\query$ be a mixed CQ (or DQ). Then $\game$ is determined under $\query$ if $X_0(\query) \in \pcurves'$.
%\end{theorem}


The value iteration update $F$ from Equation \eqref{eq:cqvi} for conjunctive queries with the standard semantics (``\Achiever\ fixes first'') can be recovered from $\uviop$ (Equation~\ref{eq:uv}) by applying intersections after each update. Formally, for all $X \in \pcurves^S$ we have
\begin{equation}
    \label{eq:observation}
    F(X) = \intersectpw \uviop(\{X\}),
\end{equation}
where $\bigcap$ is applied point-wise to all $\uviop(\{X\})_s$, $s \in S$.

%Note that the value iteration update $F$ for conjunctive queries can be recovered from $\uviop$ by applying intersections after each update. Formally, $F(X) = \bigcap \uviop(\{X\})$, where $\{X\}$ denotes the element $X \in \pcurves^S$ lifted to $\pset{\pcurves}^S$ as required by $\uviop$ and $\bigcap$ is applied point-wise. If $\bigcap \uviop(\mathcal{X}) = \uviop(\bigcap \mathcal{X})$
We will now derive a sufficient criterion for determinacy based on observation \eqref{eq:observation}. The idea is to identify a set of conditions guaranteeing that the ``final'' intersection in Lemma~\ref{lem:uvicorrect} can be ``pulled into'' the iteration, applying it after each step and thereby effectively iterating $F$.
In the next theorem we assume w.l.o.g.\ that each state $s \in S$ has exactly two successors $s_1$ and $s_2$.

\begin{theorem}
    \label{thm:det-sufficient-cond}
    Let $\mathcal{X} \in \pset{\pcurves}^S$ be such that $\uviop(\mathcal{X})_s \subseteq \mathcal{X}_s$ for all $s \in S$, where $\uviop$ is like in~\ref{eq:uv}. Further let $X^0(\query) \inpw \mathcal{X}$ and suppose that for all $s \in \Smax \cup \Sprob$ and $i \in \{0,1\}$,
    \begin{enumerate}
        \item $\mathcal{X}_{s_i}$ is closed under finite intersections of its polyhedra;
    \end{enumerate}
    and moreover, for all $X \in \mathcal{X}_{s_i}$, $X', X'' \in \mathcal{X}_{s_{1-i}}$,
    \begin{enumerate}
        \item[2)] $\conv(X \cup X') \cap \conv(X \cup X'') = \conv(X \cup (X' \cap X''))$;
        \item[3)] $(p X + \overline{p}X') \cap (pX + \overline{p}X'') = (p X + \overline{p}(X' \cap X''))$,
    \end{enumerate}
    where $p = P(s,s_{i})$ and $\overline{p} = 1-p$ in condition (3).
    Then $\game$ is determined for $\query$.
\end{theorem}
\begin{proof}[Proof (sketch)]
    For $\mathcal{Y}, \mathcal{Z} \in \pset{\pcurves}^S$ define $\mathcal{Y} \orderuvi \mathcal{Z}$ iff $\mathcal{Y}_s \subseteq \mathcal{Z}_s$ for all $s \in S$. Clearly, $\orderuvi$ is a partial order on $\pset{\pcurves}^S$ and $\uviop$ is monotone w.r.t.\ $\orderuvi$. Thus the assumptions $\mathcal{X}^0 \orderuvi \mathcal{X}$ and $\uviop(\mathcal{X}) \orderuvi \mathcal{X}$ together imply $\uviop^k(\mathcal{X}^0) \orderuvi \mathcal{X}$ for all $k \geq 0$.
    
    Let $\mathcal{X}' \orderuvi \mathcal{X}$ be such that $\mathcal{X}'_s$ is a finite set of polyhedra for all $s \in S$. The goal is to show that
    \begin{equation}
        \label{eq:to-show}
         \intersectpw \uviop(\mathcal{X}') = \intersectpw \uviop(\intersectpw \mathcal{X}')~.
    \end{equation}
    In \eqref{eq:to-show}, the intersections are applied point-wise, that is $(\intersectpw \mathcal{X}')_s \eqdef \{\bigcap \mathcal{X}'_s\}$.
    Equation~\eqref{eq:to-show} together with observation \eqref{eq:observation} implies $\intersectpw \uviop^k(\mathcal{X}^0) = F^k(X^0)$ for all $k \geq 0$ by induction. By Lemma~\ref{lem:uvicorrect}, this means that the horizon-$k$ Pareto curves are \emph{exactly the same} for all $k \geq 0$ and all initial states, yielding the overall result of the theorem.
    The remaining preconditions 1)-3) of the theorem altogether ensure that \eqref{eq:to-show} holds (see Appendix~\ref{app:proof-det-crit}).
  
%    We now show \eqref{eq:to-show}.
%    First note that we can apply the distributive law from condition 2) repeatedly to obtain the following:
%    For all $s \in \Smax$,
%    \[
%        \bigcap_{X_1 \in \mathcal{X}_{s_1}, X_2 \in \mathcal{X}_{s_2}} \conv(X_1 \cup X_2) = \conv(\bigcap \mathcal{X}_{s_1} \cup \bigcap \mathcal{X}_{s_2})~.
%    \]
%    Here we have also used condition 1).
%    A similar equation holds for the convex combination operation ($s \in \Sprob$) using 3):
%    For all $s \in \Sprob$,
%    \[
%        \bigcap_{X_1 \in \mathcal{X}_{s_1}, X_2 \in \mathcal{X}_{s_2}} (pX_1 + \overline{p}X_2) = p \bigcap \mathcal{X}_{s_1}+ \overline{p}\bigcap \mathcal{X}_{s_2}~.
%    \]
%    To show \eqref{eq:to-show}, we make a case distinction:
%    \begin{itemize}
%        \item $s \in \Smax$:\\
%        $\bigcap \uviop(\mathcal{X}')_s = \bigcap_{X_1 \in \mathcal{X'}_{s_1}, X_2 \in \mathcal{X'}_{s_2}} \conv(X_1 \cup X_2) = \conv(\bigcap \mathcal{X'}_{s_1} \cup \bigcap \mathcal{X'}_{s_2}) = \uviop(\intersectpw \mathcal{X}')_s=(\bigcap \uviop(\intersectpw \mathcal{X}'))_s$
%        \item $s \in \Smax$:\\
%        $\bigcap \uviop(\mathcal{X}')_s = \bigcap_{X_1 \in \mathcal{X}_{s_1}, X_2 \in \mathcal{X}_{s_2}} (pX_1 + \overline{p}X_2) = p \bigcap \mathcal{X}_{s_1}+ \overline{p}\bigcap \mathcal{X}_{s_2} =\uviop(\intersectpw \mathcal{X}')_s=(\bigcap \uviop(\intersectpw \mathcal{X}'))_s$
%        \item $s \in \Smin$:\\
%        $\bigcap \uviop(\mathcal{X}')_s = \bigcap (\mathcal{X}'_{s_1} \cup \mathcal{X}'_{s_2}) = \bigcap (\bigcap \mathcal{X}'_{s_1} \cup \bigcap \mathcal{X}'_{s_2})$ $=(\bigcap \uviop(\intersectpw \mathcal{X}'))_s$
%    \end{itemize}
\end{proof}

We now discuss several example applications of Theorem~\ref{thm:det-sufficient-cond}. First note that determinacy of the whole class of single-dimensional (simple) stochastic games is implied by letting \[
\mathcal{X}_s \eqdef \{[0,x] \mid x \in [0,1]\}\]
for all $s \in S$ and noticing that taking convex union and intersection of intervals of the above form is nothing but taking maximum resp.\ minimum of the upper boundaries. Since for all $x,x',x'', p \in [0,1]$,
\begin{align*}
    \min(\max(x, x'), \max(x, x'')) &= \max(x, \min(x', x'')) \\
    \min(px + \overline{p}x', px + \overline{p}x'') &= px + \overline{p}\min(x', x'')
\end{align*}
the premises of Theorem~\ref{thm:det-sufficient-cond} are all satisfied, implying determinacy of single-objective games.

Next we consider a multi-objective example:

%With Theorem~\ref{thm:det-sufficient-cond}, it is not difficult to see that Example~\ref{ex:det-crit} can be generalized as follows:
\begin{corollary}
    \label{cor:det-easy-peasy}
    Let $\game$ be a game such that no $s \in \Smax \cup \Sprob$ can reach a state $t \in \Smin$ in the game graph. Then $\game$ is determined for any mixed DQ or CQ.
\end{corollary}
\begin{proof}
    Fix any query and take $\mathcal{X} \eqdef\lim_{k \to  \infty}\uviop^k(\mathcal{X}^0)$ as the certificate in  Theorem~\ref{thm:det-sufficient-cond}. Note that for all $s \in \Smax \cup \Sprob$, we have $|\mathcal{X}_s| = 1$. The other preconditions 1)-3) of Theorem~\ref{thm:det-sufficient-cond} are thus trivially satisfied, yielding	 determinacy.
\end{proof}
For instance, the game from Figure~\ref{fig:det-strat-mem-example} is determined for all CQ and DQs, and for the particular DQ from Example~\ref{ex:det_strat_mem} the Pareto set is $\dwc(1,\nicefrac{1}{2}) \cup \dwc(\nicefrac{1}{2},1)$.
Corollary~\ref{cor:det-easy-peasy} has a simple intuitive explanation: If all of \Spoiler's choices have to take place \emph{before} any choice of \Achiever, then she does not benefit from knowing \Spoiler's strategy in advance as she can simply \emph{observe} his choices during the play. Therefore, the order of quantification is irrelevant, i.e.\ the game is determined.

The following is yet another example for an application of Theorem~\ref{thm:det-sufficient-cond}:

%As an application of the upper VI algorithm, we briefly consider determinacy of \emph{deterministic} games ($\Sprob = \emptyset$) but where randomization in strategies is still allowed. Note that $U^k(s) = L^k(s)$, where $L^k(s)$ is the lower Pareto curve at $s$ implies that the game is determined. With the help of the characterization from Thm. above we can show that
\begin{corollary}
    \label{cor:determinacy-det-game}
    Deterministic games with general strategies are determined for all mixed CQs and DQs with $n \leq 2$ objectives. For $n\geq  3$ they are not determined in general.
\end{corollary}
\begin{proof}[Proof (sketch)]
    For all $s \in S$ let $\mathcal{X}_s$ be the set of the five polyhedra depicted in Figure~\ref{fig:possible_curves}. Clearly, $\mathcal{X}^0_s \subseteq \mathcal{X}_s$ for all possible $\mathcal{X}^0$. Moreover, it is readily verified that this set of curves is closed under convex unions and intersections and that convex union distributes over intersection in the way required by Theorem~\ref{thm:det-sufficient-cond}. Thus all its preconditions are satisfied.
    
    See Appendix~\ref{app:proof_cor_det_games_n3} for an example of a deterministic game with a 3-dimensional query that is not determined.
    
%    It remains to show that deterministic games are not determined for $n \geq 3$ objectives. Therefore consider the game depicted in Figure \ref{fig:deterministic_not_determined} along with the CQ $\query = \bigwedge_{i=1}^n \probability(\reach T_i) \geq x_i$.
%    We claim that \Achiever\ has no achieving strategy for $\vec{x} = (\nicefrac{1}{2},\nicefrac{1}{2},\nicefrac{1}{2})$ if she has to fix her strategy before \Spoiler. Suppose that $\maxstrat$ is such a strategy. Then in $s_0$, $\maxstrat$ must go to the $T_3$-state with probability at least $q \geq \nicefrac{1}{2}$. Let $p$ be the probability with which $\maxstrat$ chooses to go to $T_1$ when in state $s_1$. Now consider a counter-strategy $\minstrat$ which in $T_3$ selects (i) $T_1$ with probability $1$ if $p \geq \nicefrac{1}{2}$ and (ii) $T_2$ with probability $1$ if $p < \nicefrac{1}{2}$. Then in case (i), the probability to reach $T_2$ from $s_0$ is only $(1-q) \cdot (1-p) \leq \nicefrac{1}{4}$. Similarly, in case (ii) the probability to reach $T_1$ from $s_0$ is $(1-q)\cdot p < \nicefrac{1}{4}$.
%    %    
%        To prove that the game is not determined, we show that \Spoiler\ can also not spoil the vector $\vec{x}$, assuming that he has to fix his strategy first. Therefore let $\minstrat$ be any strategy of \Spoiler.
%        It suffices to consider the two possible deterministic strategies. Consider a counter-strategy $\maxstrat$ of \Achiever\ that in $s_1$ does the opposite of what $\minstrat$ does in the $T_3$-state and plays both options with equal probability in $s_0$. Then $\maxstrat$ achieves all three targets with probability $\nicefrac{1}{2}$. Thus the game is not determined.
\end{proof}

\begin{figure}[htb]
    \centering
    \begin{tikzpicture}[scale=1.75]
    \node[scale=.75] at (0,0) (C0) {\tikz{
            \drawaxes
            \filldraw (0,0) circle (\curvedotsize)
    }};		
    \node[scale=.75] at (1,0) (C1) {\tikz{
            \drawaxes
            %\filldraw (0,1) circle (\curvedotsize);
            \draw[pcurve,very thick] (0,1) -- (0,0);
    }};	
    \node[scale=.75] at (2,0) (C2) {\tikz{
            \drawaxes
            %\filldraw (1,0) circle (\curvedotsize);
            \draw[pcurve,very thick] (1,0) -- (0,0);
    }};		
    \node[scale=.75] at (3,0) (C3) {\tikz{
            % draw in good order
            \fill[black!15] (0,0) -- (0,1) -- (1,0)-- cycle;
            \draw[pcurve] (0,1) -- (1,0);
            \drawaxes
    }};		
    \node[scale=.75] at (4,0) (C4) {\tikz{
            \fill[black!15] (0,0) -- (0,1) -- (1,1) -- (1,0)-- cycle;
            \draw[pcurve] (0,1) -- (1,1)-- (1,0);
            \drawaxes
    }};
    
    %    \node[below=0 of C0] {$D_0$};
    %    \node[below=0 of C1] {$D_1$};
    %    \node[below=0 of C2] {$D_2$};
    %    \node[below=0 of C3] {$D_3$};
    %    \node[below=0 of C4] {$D_4$};
    \end{tikzpicture}
    \caption{The five polyhedra occurring in two-dimensional deterministic games under general (randomized) strategies.}
    \label{fig:possible_curves}
\end{figure}




%Table~\ref{tab:determinacy} summarizes determinacy of deterministic and stochastic games with deterministic or general strategies 
%\begin{table}[htb]
%    \centering
%    \caption{Necessary and sufficient conditions for general determinacy in terms of the number $n$ of objectives.}
%    \label{tab:determinacy}
%    \begin{tabular}{l  c c}
%        \toprule
%        & \multicolumn{2}{c}{\emph{Strategies}} \\
%        \emph{Game} & \emph{Deterministic} & \emph{General} \\
%        \midrule
%        \emph{Deterministic} & $n \in \mathbb{N}$~\cite{FH10} & $n \leq 2$ [Cor.~\ref{cor:determinacy-det-game}]\\
%        \emph{Stochastic} & $n = 1$~\cite{Condon92} & $n = 1$~\cite{CFK+13}\\
%        \bottomrule    
%    \end{tabular}
%\end{table}

For expected reward objectives as considered e.g.\ in \cite{cfk13}, the proof of Corollary~\ref{cor:determinacy-det-game} does not work because there are more (infinitely many) possible Pareto sets than the ones from Figure~\ref{fig:possible_curves} which do not satisfy condition 2) from Theorem~\ref{thm:det-sufficient-cond}.

Finally, we remark that Theorem~\ref{thm:det-sufficient-cond} asserts a strong notion of determinacy---namely that the game is determined for \emph{all} finite horizons $k \geq 0$ (and thus for infinite horizon as well). However, it is not hard to find examples of games that are not determined for some finite horizon $k < \infty$ but become determined at $k{+}1$. Thus, Theorem~\ref{thm:det-sufficient-cond} is not a necessary condition for determinacy 

\subsection{Decision procedure for determinacy}\label{sec:determDecProc}

Finally, using a recent result from \cite{lics-mosg}, we can show that determinacy is decidable for reachability CQs or safety DQs, even for non-stopping games. This extends a result of~\cite{BF16}. \cite{lics-mosg} presents a value iteration which, given a reachability CQ $\query$ has the Pareto set $\val(\game,\query)$ as its \emph{unique} fixpoint.
To decide determinacy, we compute the \emph{exact} set $\upval(\game,\query)$ and verify that it is a fixpoint, implying $\upval(\game,\query) = \val(\game,\query)$; and similar for safety DQs which we can recast into reachability CQs as described in Section~\ref{sec:alg_vi}. Thus:

%We extend the decision procedure for determinacy of stopping SGs with total reward queries to arbitrary SGs with safety disjunctive queries or reachability conjunctive queries.
%The set of vectors $X$ that \Achiever\ can achieve for a safety DQ are exactly those that \Spoiler\ cannot achieve for a reachability CQ with the same target sets under the \enquote{will-know} semantics, by recasting the query as described in Section~\ref{sec:alg_vi}. 
%Thus, $\overline{X} = [0,1]^n \setminus X$ is an over-approximation of the set of threshold vectors that \Spoiler\ can achieve for a reachability CQ under standard semantics. Moreover, in the case of determinacy, $\overline{X}$ is equal to the achievable vectors under standard semantics. 
%We combine this with the value iteration procedure from~\cite{lics-mosg}, which, given a CQ, has the unique fixpoint of the achievable vectors under standard semantics. 
%So if $\overline{X}$ is a fixpoint of the value iteration, we know that the CQ is equal under standard and will-know semantics.
%On the other hand, if we apply one iteration of the procedure from~\cite{lics-mosg} and the set becomes smaller, we know $\overline{X}$ was an over-approximation and can infer that the SG with the CQ is not determined. 
%
%Thus, the procedure is as follows: Given an SG and either a CQ or a DQ, we also construct the other (recast) query.
%Then we compute the achievable vectors for the DQ $X$ by any algorithm previously mentioned in the paper.
%Finally, we perform one step of the value iteration from~\cite{lics-mosg} on the set $\overline{X} =  [0,1]^n \setminus X$.
%The SG with the queries is determined if and only if $\overline{X}$ is a fixpoint of this value iteration.

\begin{theorem}
    Given an SG and a reachability CQ or safety DQ $\query$, it is decidable if $\game$ is determined for $\query$.
\end{theorem}

%Thus, given a safety DQ, we can check determinacy by computing the complement of the achievable vectors $\overline{X} = \mathbbm{1} \setminus X$ and 
%
%The safety values of a DQ that \Achiever can ensure are exactly those that \Spoiler cannot reach in a conjunctive query under the 
%Further, the points \Spoiler can reach under the \enquote{will-know} semantics are a superset of those he can reach under standard semantics, and equal if the SG is determined.
%We use this to check determinacy as follows:
%
%(i) Compute the safety values of the DQ.
%(ii) Let $X$ be the complement of these values, i.e. those that \Spoiler can reach  under \enquote{will-know} semantics.
%(iii)  
%For a conjunctive query under standard semantics, the modified Bellman operator of~\cite{lics-mosg} has the unique fixpoint of the 
% can be over-approximated by the points that \Spoiler can definitely not reach. 
%Formally, this is proven by considering 
%Further, in the case of determinacy, the two sets are equal.
%Formally:
%
%
%\todot{make shorter, present as a corollary to lics20 and not as a huge new result. only talk about reach to be on the safe side}
%
%In this section, we will relate the sets of achievable points for DQs and CQs. Thus, we recall and modify the definition of the set of achievable points as follows:
%For an SG $\G$ and a vector of objectives $\vec{T}$ we have
%\begin{align*}
%\val_{D}(\G,\vec{T}) &\eqdef \{x \mid \exists \straa \forall \strab \exists i \colon \probability^{\straa,\strab}(\genobj_i T_i) \geq x_i \}\\
%\val_{C}(\G,\vec{T}) &\eqdef \{x \mid \exists \strab \forall \straa \forall i \colon \probability^{\straa,\strab}(\genobj_i T_i) > x_i \}
%\end{align*}
%Note that we added an index to indicate whether the points are achievable for a CQ or a DQ. Also, to simplify the proofs, for the CQ $\strab$ denotes the strategy of $\Achiever$ and $\straa$ of $\Spoiler$. 
%Further, we denote by $\mathbbm{1}$ the hypercube of all possible achievable points, the downward closure of the point with $1$ in every dimension.
%Finally, let $\vec{\neg T}$ be the inversion of the objectives in $T$, i.e.\ every $\genobj_i T_i$ is replaced by $\overline{\genobj_i T_i}$.
%
%\begin{lemma}\label{lem:invert}
%	For any SG $\G$ and objective vector $\vec{T}$ it holds that
%	\[\val_{C}(\G,\vec{T}) \subseteq (\mathbbm{1} \setminus \val_{D}(\G,\vec{\neg T}))\]
%	Further, the two sets are equal if and only if $\G$ with the CQ $\vec{T}$ or the DQ $\vec{\neg T}$ is determined.
%\end{lemma}
%\begin{proof}
%	Intuitively, the points that can be achieved by the CQ are those points that the opponent cannot spoil in any way. 
%	The latter can be approximated by the points that the opponent can spoil against all achieving strategies, which is a DQ.
%	All points without those in the DQ are an over-approximation of the achievable points. 
%	In the case that the SG with the query is determined, all points without the spoilable points are exactly the achievable points.
%	
%	Formally, we have 
%	\begin{align*}
%		\val_{C}(\G,\vec{T})
%		&\eqdef \{x \mid \exists \strab \forall \straa \forall i \colon \probability^{\straa,\strab}(\genobj_i T_i) > x_i \}\\
%		&= \mathbbm{1} \setminus \{x \mid \forall \strab \exists \straa \exists i \colon \probability^{\straa,\strab}(\overline{\genobj_i T_i}) \geq x_i \} \tag{negating the query}\\
%		& \subseteq \mathbbm{1} \setminus \{x \mid \exists \straa \forall \strab  \exists i \colon \probability^{\straa,\strab}(\overline{\genobj_i T_i}) \geq x_i \} \tag{exchanging quantors}\\
%		& = \val_{D}(\G,\vec{\neg T})		
%	\end{align*}
%	Note that 
%	\[
%	\{x \mid \forall \straa \exists \strab \exists i \colon \probability^{\straa,\strab}(\overline{\genobj_i T_i}) > x_i \} \supseteq \{x \mid \exists \strab \forall \straa  \exists i \colon \probability^{\straa,\strab}(\overline{\genobj_i T_i}) > x_i \},
%	\]
%	so when exchanging quantors the set we subtract becomes smaller and thus the comparator is $\subseteq$.
%	
%	In the case of determinacy, the two sets are equal. Then instead of $\subseteq$ we have equality.
%\end{proof}
%
%We use Lemma~\ref{lem:invert} to decide determinacy as follows:
%Given an SG $\G$ and a CQ with objective vector $\vec{T}$, we compute $\val_{D}(\G,\vec{\neg T})$, using any of the algorithms described in this paper.
%To check whether $\val_{D}(\G,\vec{\neg T}) = \val_{C}(\G,\vec{T})$, we utilize the modified Bellman  operator $\mathcal{B}$ of the value iteration procedure from~\cite{lics-mosg}. 
%Its unique fixpoint is $\val_{C}(\G,\vec{T})$. \todo{actually with $\geq$, not $>$}
%So if $\mathcal{B}(\val_{D}(\G,\vec{\neg T})) = \val_{D}(\G,\vec{\neg T})$, the SG with the CQ is determined, and otherwise it is not.
%
%Note that $\mathcal{B}$ is only defined for reachability CQs. For safety CQs, we need the following:
%\begin{lemma}
%	For an SG $\G$ and a CQ with objective vector $\vec{T}$ where all objectives are safety, 
%	$\val_{C}(\G,\vec{T})$ is the greatest fixpoint of the multi-objective Bellman equations of~\cite{cfk13}.
%\end{lemma}
%\begin{proof}
%	None of my ideas worked so far.
%\end{proof}
%
%If this Lemma was true, we could just apply the multi-objective Bellman equations of~\cite{cfk13} once.
%This is because $\val_{C}(\G,\vec{T})$ is the greatest fixpoint of the multi-objective Bellman equations and $\val_{D}(\G,\vec{\neg T}) \supseteq \val_{C}(\G,\vec{T})$, so if it does not decrease, we know we found the fixpoint.
%
%For mixed CQs, we conjecture that, since the modifications of~\cite{lics-mosg} are sound, stuff magically works out.
%
%For checking the determinacy of an SG and a DQ with objective vector $\vec{T}$, we check the determinacy of the inverted CQ with objective vector $\vec{\neg T}$.









%Intuitively, if an SG with a multi-objective query is determined, then the points that one player can achieve for a query are exactly those points that the opponent cannot spoil.
%Otherwise, there are points that are neither certainly achievable nor certainly spoilable. 
%Thus, asking which points the opponent certainly cannot spoil is an over-approximation of the points that are achievable. 
%
%For CQs, we can use the value iteration procedure from~\cite{lics-mosg} to check wether some given set of points is the set of achievable points.
%








%First, we argue how to check determinacy of an SG and a CQ. We will argue how to check determinacy of DQs afterwards.
%For CQs, there exists an extension of value iteration that has the unique fixpoint of the achievable points~\cite{lics-mosg}.
%That means that, given a set of points it returns a set of points; and the two are equal if and only if the input is the set of achievable points for the CQ.
%
%Using this, we can check determinacy of an SG with a given CQ as follows:
%\begin{itemize}
%	\item Compute the points that the opponent can certainly spoil, i.e.\ invert the query and compute the points that the opponent can certainly achieve.
%	\item Let $X$ be the set of all points that are not certainly spoilable. $X$ is an over-approximation of the achievable points. 
%	\item The SG with this CQ is determined if and only if $X$ is the fixpoint of the value iteration procedure. 
%\end{itemize}
%
%\begin{theorem}
%	An SG $\G$ with a reachability- or safety-CQ is determined if an only if 
%\end{theorem}
%
%Game is determined if
%\begin{align*}
%	\frontier(s,\genobj,DQ) =\\
%	\{x \mid \forall \strab \exists \straa \exists i \colon \probability^{\straa,\strab}(\genobj_i T_i) \geq x_i \} = \tag{exchanging quantors}\\
%	 \mathbbm{1} \setminus \{x \mid \exists \strab \forall \straa \forall i \colon \probability^{\straa,\strab}(\genobj_i T_i) < x_i \} = \tag{inverting frontier}\\
%	 \mathbbm{1} \setminus \{x \mid \exists \strab \forall \straa \forall i \colon \probability^{\straa,\strab}(\overline{\genobj_i} T_i) \geq x_i \} = \tag{inverting objective}\\
%	 \mathbbm{1} \setminus \frontier(s,\overline{\genobj},CQ)\tag{with players exchanged}
%\end{align*}
%
%So given an objective and a DQ, we have to check that it is equal to the solution of hypercube minus the inverted CQ; or for a CQ we check that it is equal to hypercube minus the inverted DQ.
%If it was not determined, then the first line equal becomes a $\subseteq$, by way of exchanging quantors, since $\exists \forall$ implies $\forall \exists$ but not vice versa. 
%So the DQ-frontier is certainly a subset. 1 - DQ-frontier is certainly larger. We only have to check whether it is equal to the CQ.
%We can take the 1-DQ-frontier as over-approximation of the CQ-frontier and then use a procedure that given a CQ and an over-approximation converges towards the CQ-frontier. If DQ-frontier is a fixpoint, we know they are equal. If the procedure makes it smaller, the game is not determined. 
%For reachability CQ, \cite{lics-mosg} gives such a procedure.
%For safety CQ, the value iteration from \cite{cfk13} is such a procedure for over-approximations. We prove this here:

%\begin{lemma}
%	Given an SG, a safety CQ and an over-approximation of the frontier, the MO-Bellman equations converge towards the true frontier.
%\end{lemma}
%\begin{proof}
%	\begin{enumerate}
%		\item The true frontier is a fixpoint of the MO-Bellman equations.
%		\begin{itemize}
%			\item I can invert to asking a reachability question. 
%			\item For this, by \cite{cfk13} we know it is a fixpoint.
%		\end{itemize}
%		\item It is indeed the greatest fixpoint of the MO-Bellman equations where the avoid states have value 0. 
%		\begin{itemize}
%			\item Replay the proof of Prop 5.3 from lics-mosg until step 6 (since all the notions are the same and it is independent from deflating).
%			\item X contains an EC $X'$. This EC cannot have value 1, so there is a Minimizer exit with lower value. Consider this Minimizer exit. If it leads to another state in $X$, then consider the subset of $X$ that is reachable from the successor of the state that is not in $X'$ and repeat the process. At some point, we reach a bottom EC that has no successors inside $X$. Then this exit has to lead outwards, and thus we get a contraction, and thus a contradiction.
%		\end{itemize}
%		\begin{itemize}
%			\item Assume for contradiction we have a greater fixpoint. Let $X$ be the set of states with greatest difference.
%			\item $X$ contains no avoid states and no states with frontier $\mathbbm{1}$, since they all have a difference of 0.
%			\item An exiting action is contracting, so no state in $X$ depends on a leaving action.
%			\item 
%		\end{itemize}
%	\end{enumerate}
	
	
%	The k-step upper safety frontier is 1 - the k-step reach frontier with players exchanged. 
%	\begin{align*}
%		\{x \mid \exists \straa \forall \strab \forall i \colon \probability^{\straa,\strab}(\safe_i T_i) > x_i \}\\
%		= \mathbb{1} \setminus \{x \mid \forall \straa \exists \strab \exists i \colon \probability^{\straa,\strab}(\safe_i T_i) \leq x_i \} \\
%		= \mathbb{1} \setminus \{x \mid \forall \straa \exists \strab \exists i \colon \probability^{\straa,\strab}(\reach_i T_i) > x_i \} \\
%	\end{align*}
%	Seems this doesn't really work...
%	
%	Another idea, like the proof of Theorem 4 in CFK+13 (concretely Appendix B.3 in the extended version): 
%	By induction, we show that the k-step safety frontier from above is exactly the k-step safety value (define what exactly I mean by that).
%	Thus, in the limit we get the right value. 
%\end{proof}
%So the procedure to decide whether a game with a DQ or a CQ is determined is:
%1. Get both the CQ and the DQ by inverting.
%2. Compute $\mathbbm{1} \setminus \frontier(s)$ for the DQ
%3. On this, do one step of MO-Bellan and, if CQ is reach, one MO-Deflate.
%It can't increase. If it decreased, the game is not determined. If it didn't change, the game is determined. 

%
%A game is determined iff DQ ex forall frontier = DQ forall ex frontier. 
%The DQ forall ex frontier is the opposite of the CQ ex forall frontier. 
%We have a procedure that given an over-approximation of the CQ ex forall frontier (which the DQ ex forall frontier is) has only a single fixpoint, namely the CQ ex forall frontier. 
%So by computing the DQ ex forall frontier and then applying the VI from LICS20, we know whether a game is determined. If yes, we have also found the unique frontier.
%
%\begin{align*}
%\frontier(s) &\eqdef \{x \mid \exists \straa \forall \strab \exists i \colon \probability^{\straa,\strab}(\genobj_i T_i) \geq x_i \}\\
%&\subseteq \{x \mid \forall \strab \exists \straa \exists i \colon \probability^{\straa,\strab}(\genobj_i T_i) \geq x_i \} \tag{equal if determined}\\
%&= \mathbbm{1} \setminus \{x \mid \exists \straa \forall \strab \forall i \colon \probability^{\straa,\strab}(\genobj_i T_i) < x_i \} \\
%\end{align*}
%
%$\mathbbm{1} \setminus \frontier(s)$ is an over-approximation of $\{x \mid \exists \straa \forall \strab \forall i \colon \probability^{\straa,\strab}(\genobj_i T_i) < x_i \}$. If they are equal, the game is determined. 
%
%Given an over-approximation of a CQ, we can use the procedure from LICS 20 to check whether it is a fixpoint. 
%If all objectives are reachability, this works out of the box.
%If all objectives are safety, then here is a proof that the MO-bellman equations are a contraction.

%

%
%However, we have to modify it to deal with safety and strict less than. 
%Actually, safety less than is reachability greater than, so that works the same way.
%Reachability less than should work, because for safety upper bounds converge from above (and we need inflating). However, I'm unsure how to show this for MOSG, and even more unsure about mixture, and even more unsure since actually the procedure is undefined for what I use it for here.

%\subsection{Overapproximation in games that are not determined}
%The DQ ex forall frontier certainly is an over-approximation of the CQ ex forall frontier. It is tighter than just checking all objectives, see example. 
%So given a CQ ex forall question, where one expects a negative answer, instead of using the VI with uncertain convergence time, one can also use DQ ex forall frontier as a quick test.
%[probably just drop this, even I am not convinced...]

%Besides the interest in DQs themselves, they can be used to over-approximate the outcome of certain CQs and inside the decision procedure whether a game is determined. 
%
%Start with example, show that safety query implies that other player cannot achieve conjunction of reach. Have one determined and one undetermined game.
%
%Let $\overline{\genobj}$ denote the inversion of an objective.
%
%\begin{align*}
%		 	   & \exists \straa \forall \strab \colon \bigvee_{i=1}^n \probability^{\straa,\strab}(\genobj_i T_i) \geq x_i\\
%	\iff 	   & \neg (\forall \straa \exists \strab \colon \bigwedge _{i=1}^n \probability^{\straa,\strab}(\genobj_i T_i) < x_i)\\
%	\impliedby & \neg (\exists \strab \forall \straa \colon \bigwedge _{i=1}^n \probability^{\straa,\strab}(\genobj_i T_i) < x_i)
%\end{align*}
%In the second line, we added to negations and pulled one in. In the third line, we changed the order of the quantors.
%
%By contraposition and inverting the objective instead of the comparator, we get:
%\begin{align*}
%			 & \neg \exists \straa \forall \strab \colon \bigvee_{i=1}^n \probability^{\straa,\strab}(\genobj_i T_i) \geq x_i\\
%	\implies & \exists \strab \forall \straa \colon \bigwedge _{i=1}^n \probability^{\straa,\strab}(\overline{\genobj_i} T_i) > x_i
%\end{align*}
%
%Thus, when given a CQ, we can use a DQ to get a negative answer. 
%A conjunction is achievable only if the other player cannot spoil any of the objectives. 
%Note that this test is stronger than just checking all single objectives, see example.
%
%Additionally, if the game is determined as in other example, then the $\implies$ actually is an $\iff$, so we can answer CQs by answering DQs. However, to the best of our knowledge DQs are a lot simpler, as we have a decision procedure for them (and provide better algos in this paper).
%





%
%Asking whether a DQ is achievable for one player gives an over-approximation of which points of an inverted CQ of the other player could achieve.
%Thus, we can use a DQ to over-approximate CQs (as in BF16, Sec 3).
%Note that this is tighter than just solving all targets alone, as e.g. in this example (if one player is missing and the curve is not the hypercube).
%
%
%
%
%
%Determinacy:
%- In determined games, CQ and DQ are same, because we can invert like this.
%- So if we solve DQ, we get the value.
%- To check whether game is determined, we can solve DQ (thus get over-approximation of CQ val), and then do MO-DEFLATE step and check whether any value decreases. By LICS20, if CQ neq DQ, something decreases. If decrease, then not determined. If no decreases, then determined and we have the value.
%
%Maxi.
%
%Table 3.2 [TW]: Does determinacy come from rand strat or rand game? Both.
%
%\textcolor{red}{More on determined games: What kind of properties do they have, how do they look, when is a game determined? Maybe get some info from UV solutions?}
%
%
%Given a determined SG, we can just compute the upper value (e.g. by considering all memoryless deterministic strategies, or by some cool algo in this paper); however, if we don't know whether the game is determined, we need some way to verify that this upper value is indeed also the lower value.
%In \cite[Sec. 3]{BF16}, the authors suggest a solution for stopping games. We extend this to general games as follows:
%Given the upper Pareto frontier, we perform one step of the over-approximation value iteration (with MO-DEFLATE) from~\cite{lics-mosg}. Since for any over-approximation, that algorithm converges towards the true lower Pareto frontier (as that is the only fixpoint), the upper Pareto frontier will decrease in some dimension, unless the game is indeed determined.
%
%This is the first algorithm to solve arbitrary determined MOSG.
%\todomaxi{And it is really the same argument as in BF16, only that we use a different VI algo...}

%As we saw in Section \ref{sec:alg_vi}, we can invert a DQ to an equivalent CQ and vice versa as follows:
%\begin{align*}
%	& \neg \exists \maxstrat \forall \minstrat \bigvee_i \probability(\genobj_i T_i) \geq x_i \\
%	%\iff \quad & \forall \maxstrat \exists \minstrat \bigwedge_i \probability(\genobj_i T_i) < x_i \\
%	\iff \quad &  \forall \maxstrat \exists \minstrat \bigwedge_i \probability(\overline{\genobj_i T_i}) > 1 - x_i~.
%\end{align*}
%
%If an SG with a certain query is determined, we also can exchange the order of the quantors in front of the query, and thus we get
%\begin{align*}
%	& \neg \exists \maxstrat \forall \minstrat \bigvee_i \probability(\genobj_i T_i) \geq x_i \\
%	%\iff \quad & \forall \maxstrat \exists \minstrat \bigwedge_i \probability(\genobj_i T_i) < x_i \\
%	\iff \quad &   \exists \minstrat \forall \maxstrat \bigwedge_i \probability(\overline{\genobj_i T_i}) > 1 - x_i~.
%\end{align*} 
%Thus, in determined SGs, the sets of achievable points relate as follows: The points that can be achieved for a CQ by one player are exactly the points that the opponent cannot spoil, i.e. all achievable points (the hypercube $\mathbbm{1}$) without the points that the opponent can achieve in the negated DQ.
%
%Define in prelims, noting that any CQ or DQ can be brought into this form by turning all objectives such that we have a geq question (ignoring strictness and mixtures):
%\begin{align}
%	\frontier(s,\vec{\genobj},DQ) &\eqdef \{x \mid \exists \straa \forall \strab \exists i \colon \probability^{\straa,\strab}(\genobj_i T_i) \geq x_i \}\\
%	\frontier(s,\vec{\genobj},CQ) &\eqdef \{x \mid \exists \straa \forall \strab \forall i \colon \probability^{\straa,\strab}(\genobj_i T_i) \geq x_i \}
%\end{align} 

